Adverse Health Correlates of Intimate Partner Violence against Older Women: Mining Electronic Health Records

Intimate partner violence (IPV) is often studied as a problem that predominantly affects younger women. However, studies show that older women are also frequently victims of abuse even though the physical effects of abuse are harder to detect. In this study, we mined the electronic health records (EHR) available through IBM Explorys to identify health correlates of IPV that are specific to older women. Our analyses suggested that diagnostic terms that are co-morbid with IPV in older women are dominated by substance abuse and associated toxicities. When we considered differential co-morbidity, i.e., terms that are significantly more associated with IPV in older women compared to younger women, we identified terms spanning mental health issues, musculoskeletal issues, neoplasms, and disorders of various organ systems including skin, ears, nose and throat. Our findings provide pointers for further investigation in understanding the health effects of IPV among older women, as well as potential markers that can be used for screening IPV.

==> IPV-Senior, PLoS ONE/figure2_histograms.tex <==
\begin{figure}[t]
	\centerline{
		\includegraphics[width=0.33\linewidth]{figures/histogram_ipv_senior_marked.png}
		\includegraphics[width=0.33\linewidth]{figures/histogram_ipv_bg_marked.png}
		\includegraphics[width=0.33\linewidth]{figures/histogram_differential_comorbidity_marked.png}
	}
	\caption{\textbf{The distributions of co-morbidity and differential co-morbidity scores in Senior and Background populations.} (Left \& Middle panels) The distribution of the co-morbidity scores for all terms in Senior and Background populations. The null hypothesis thresholds to determine Minor/Moderate/High co-morbidity are marked on the histograms (OR=3/5/10). (Right panel) The distribution of the differential co-morbidity scores for all terms. Since there is not a notable shift in the histogram, OR=1 is considered as the null level for differential co-morbidity.}
	\label{fig:histograms}
\end{figure}

==> IPV-Senior, PLoS ONE/figure3_regionplot.tex <==
\begin{figure}[t]
	\centerline{
		\includegraphics[width=0.55\linewidth]{figures/ipv_senior_regionplot.png}
	}
	\caption{X-axis and Y-axis indicate the minimum bounds of 95\% augmented confidence intervals (adjusted for FDR) for IPV co-morbidity scores in Senior and Background (BG) populations i.e., OR(t, IPV|Senior), and OR(t, IPV|BG) respectively. The terms identified with High/Moderate/Minor co-morbidity in both populations are shown in red/yellow/blue regions respectively. The terms identified as differentially co-morbid (having significantly higher co-morbidity in Senior population) are marked with black circles. }
	\label{fig:regionplot}
\end{figure}

==> IPV-Senior, PLoS ONE/table1_senior.tex <==
\begin{landscape}
	\begin{table}
%		\vspace{0.3cm}
		\resizebox{1\columnwidth}{!}{		
			%\center{}
			\begin{tabular}{|p{0.1cm} p{7.5cm}|cc|cccc|@{}}
				\toprule
				& \multicolumn{1}{c|}{\bf Term Description} & \multicolumn{2}{c|}{\bf Co-morbidity in Senior population} &  \multicolumn{4}{c|}{\bf Number of Records} \\
%				& \multicolumn{1}{c|}{\bf Term Description} & \multicolumn{2}{c|}{\bf OR(t, IPV$|$Senior)} &  \multicolumn{4}{c|}{\bf Number of Records} \\
				& & Raw & Adjusted & BG & IPV & Senior& SeniorIPV\\
				\hline
 1 & History of abuse & 91.4 [27.9, 299.4] H & 30.5 [9.3, 99.8] H & 36660 & 310 & 2780 & 20 \\
 \hline
 2 & Maltreatment syndromes & 194.7 [27.9, 1358.4] H & 64.9 [9.3, 452.8] H & 4390 & 100 & 660 & 10 \\
 \hline
 3 & Poisoning caused by anticonvulsant & 50.4 [16.2, 156.6] H & 16.8 [5.4, 52.2] H & 26920 & 190 & 5100 & 20 \\
 \hline
 4 & Poisoning caused by sedative AND/OR hypnotic & 46.3 [15.5, 138.3] H & 15.4 [5.2, 46.1] H & 28660 & 200 & 5650 & 20 \\
 \hline
 5 & Continuous acute alcoholic intoxication in alcoholism & 85.8 [13.7, 535.5] H & 28.6 [4.6, 178.5] H & 7870 & 120 & 1400 & 10 \\
 \hline
 6 & Continuous opioid dependence & 38.9 [12.9, 116.9] H & 13.0 [4.3, 39.0] H & 25590 & 140 & 6750 & 20 \\
 \hline
 7 & Chronic post-traumatic stress disorder & 28.2 [12.1, 65.8] H & 9.4 [4.0, 21.9] H & 136510 & 680 & 14260 & 30 \\
 \hline
 8 & History of physical abuse & 64.6 [10.8, 386.9] H & 21.5 [3.6, 129.0] H & 29000 & 290 & 1990 & 10 \\
 \hline
 9 & Poisoning caused by central nervous system drug & 21.7 [10.8, 43.6] H & 7.2 [3.6, 14.5] H & 150480 & 820 & 25370 & 40 \\
 \hline
10 & Acute drug intoxication & 29.9 [10.5, 85.0] H & 10.0 [3.5, 28.3] H & 69550 & 420 & 8690 & 20 \\
 \hline
11 & Alcohol intoxication & 29.5 [10.5, 82.6] H & 9.8 [3.5, 27.5] H & 68940 & 420 & 8650 & 20 \\
 \hline
12 & Contusion of multiple sites & 20.8 [10.5, 41.1] H & 6.9 [3.5, 13.7] H & 55570 & 850 & 26750 & 40 \\
 \hline
13 & Pathological drug intoxication & 29.4 [10.3, 84.0] H & 9.8 [3.4, 28.0] H & 70250 & 430 & 8860 & 20 \\
 \hline
14 & Posttraumatic stress disorder & 22.1 [10.0, 48.7] M & 7.4 [3.3, 16.2] M & 161610 & 720 & 17980 & 30 \\
 \hline
15 & Toxic effect of ethyl alcohol & 27.3 [9.8, 75.7] M & 9.1 [3.3, 25.2] M & 73690 & 450 & 9480 & 20 \\
 \hline
16 & Poisoning caused by chemical substance & 18.5 [9.5, 36.3] M & 6.2 [3.2, 12.1] M & 154130 & 730 & 29160 & 40 \\
 \hline
17 & Poisoning caused by psychotropic agent & 26.4 [9.5, 73.8] M & 8.8 [3.2, 24.6] M & 60390 & 360 & 9730 & 20 \\
 \hline
18 & Alcohol abuse & 16.7 [9.3, 29.9] M & 5.6 [3.1, 10.0] M & 220590 & 1200 & 42040 & 50 \\
 \hline
19 & Drug abuse & 19.8 [9.1, 43.0] M & 6.6 [3.0, 14.3] M & 190400 & 1020 & 20100 & 30 \\
 \hline
20 & Nondependent alcohol abuse & 23.6 [8.7, 63.7] M & 7.9 [2.9, 21.2] M & 36180 & 230 & 11090 & 20 \\
 \hline
			\end{tabular}
		}
		\caption{\textbf{Top 20 terms having high co-morbidity with IPV in older women population.} For each term, we report both the raw co-morbidity scores (the odds ratios) and their adjusted versions to alleviate selection bias. For each co-morbidity score, we report the following: The point estimate (odds ratio), 95\% augmented confidence interval (adjusted for FDR), and the corresponding co-morbidity level. The co-morbidity levels are abbreviated: H for high, M for moderate, and {\it m} for minor. The terms are sorted in descending order according to the minimum bound of their confidence intervals $\text{OR}_{\min}$(t, IPV$|$Senior). This table reports the top 20 terms that exhibit high (OR>>10) or moderate level of association (OR>>5) with IPV in the older women population. See Supplementary Data 2 for a full list of terms identified as significant. %All 20 reported terms are identified with high confidence. This indicates that, compared to other terms, they have higher association with IPV in a statistically significant manner in older women population.
}
		\label{table:senior}
	\end{table}	
\end{landscape}

==> IPV-Senior, PLoS ONE/table2_differential.tex <==
\begin{landscape}
	\begin{table}
	%	\vspace{0.3cm}
		\resizebox{\columnwidth}{!}{		
			%\center{}
			\begin{tabular}{|c| p{5.5cm}|cc|c|cccc|@{}}
				%			\\
				%					\hline
				%		\vspace{-1cm}
				\toprule
				%		\hline
				%		\\
				\multicolumn{1}{|c|}{\bf Category} & \multicolumn{1}{c|}{\bf Term Description} & \multicolumn{2}{c|}{\bf Adjusted Co-morbidity in Population Z} & \multicolumn{1}{c|}{\bf Differential Co-morbidity} &  \multicolumn{4}{c|}{\bf Number of Records} \\
				& & Senior & Background (BG) & {Senior vs. BG} & BG & IPV & Senior& SeniorIPV\\
				\hline
\multirow{1}{*}{Drug Interactions} & Poisoning caused by anticonvulsant & 16.8 [5.4, 52.2] H & 4.7 [3.6, 6.0] H & 3.61 [1.27, 10.25]  & 26920 & 190 & 5100 & 20 \\
 \hline
\multirow{1}{*}{Miscellaneous} & History of abuse & 30.5 [9.3, 99.8] H & 5.7 [4.6, 7.0] H & 5.38 [1.58, 18.32]  & 36660 & 310 & 2780 & 20 \\
 \hline
\multirow{2}{*}{Substance Use Issues} & Continuous opioid dependence & 13.0 [4.3, 39.0] H & 3.6 [2.7, 4.7] M & 3.64 [1.26, 10.51]  & 25590 & 140 & 6750 & 20 \\
 \cline{2-9}
 & Alcohol intoxication & 9.8 [3.5, 27.5] H & 4.1 [3.5, 4.9] H & 2.38 [1.02, 5.55]  & 68940 & 420 & 8650 & 20 \\
 \hline
\multirow{7}{*}{Mental Health} & Chronic post-traumatic stress disorder & 9.4 [4.0, 21.9] H & 3.5 [3.1, 4.0] M & 2.68 [1.24, 5.82]  & 136510 & 680 & 14260 & 30 \\
 \cline{2-9}
 & Major depression in partial remission & 5.2 [2.1, 12.8] M & 1.2 [0.9, 1.7]  & 4.30 [1.31, 14.15]  & 31750 & 60 & 16870 & 20 \\
 \cline{2-9}
 & Adjustment disorder with mixed emotional features & 3.9 [1.6, 9.5] {\it m} & 1.1 [0.9, 1.4]  & 3.62 [1.25, 10.44]  & 77440 & 130 & 22080 & 20 \\
 \cline{2-9}
 & Generalized anxiety disorder & 1.9 [1.3, 2.8] {\it m} & 1.1 [1.0, 1.2] {\it m} & 1.70 [1.10, 2.63]  & 578410 & 910 & 211620 & 80 \\
 \cline{2-9}
 & Chronic mood disorder & 1.9 [1.3, 2.9] {\it m} & 1.2 [1.1, 1.4] {\it m} & 1.55 [1.01, 2.39]  & 473480 & 830 & 176180 & 70 \\
 \cline{2-9}
 & Anxiety disorder & 1.7 [1.2, 2.3] {\it m} & 1.2 [1.1, 1.3] {\it m} & 1.40 [1.02, 1.92]  & 1718770 & 2420 & 624790 & 170 \\
 \hline
\multirow{3}{*}{Muscle Skeletal Issues} & Injury of ligament of hand & 4.9 [1.9, 12.2] M & 2.0 [1.6, 2.3] {\it m} & 2.48 [1.02, 5.98]  & 90940 & 270 & 17730 & 20 \\
 \cline{2-9}
 & Synovitis & 1.8 [1.0, 3.0] {\it m} & 0.8 [0.6, 0.9]  & 2.32 [1.19, 4.55]  & 188300 & 220 & 101300 & 40 \\
 \cline{2-9}
 & Acquired deformity of joint of foot & 1.4 [0.9, 2.2]  & 0.5 [0.5, 0.7]  & 2.64 [1.31, 5.33]  & 176850 & 150 & 159380 & 50 \\
 \hline
\multirow{4}{*}{Disorders} & Hypoglycemia & 2.1 [1.1, 3.8] {\it m} & 1.1 [0.9, 1.3]  & 1.96 [1.00, 3.86]  & 104830 & 170 & 64730 & 30 \\
 \cline{2-9}
 & Developmental disorder & 2.3 [1.0, 5.0] {\it m} & 0.8 [0.7, 0.9]  & 2.86 [1.12, 7.30]  & 425210 & 510 & 36860 & 20 \\
 \cline{2-9}
 & Nutritional disorder & 1.0 [0.8, 1.3]  & 0.5 [0.5, 0.5]  & 2.01 [1.31, 3.10]  & 1289750 & 950 & 980750 & 170 \\
 \cline{2-9}
 & Vitamin D deficiency & 0.9 [0.7, 1.2]  & 0.5 [0.4, 0.5]  & 1.99 [1.28, 3.10]  & 911940 & 640 & 669660 & 120 \\
 \hline
\multirow{1}{*}{Skin Problem} & Tinea pedis & 2.4 [1.1, 5.5] {\it m} & 0.8 [0.6, 1.0]  & 3.22 [1.15, 9.03]  & 67660 & 80 & 34850 & 20 \\
 \hline
\multirow{1}{*}{Infectious disease} & Infectious disease of lung & 1.9 [1.1, 3.2] {\it m} & 0.9 [0.7, 1.1]  & 2.09 [1.08, 4.03]  & 78290 & 110 & 96360 & 40 \\
 \hline
\multirow{1}{*}{Women's Health} & Pelvic injury & 1.8 [1.1, 3.0] {\it m} & 1.0 [0.9, 1.1]  & 1.76 [1.01, 3.07]  & 612530 & 890 & 102340 & 40 \\
 \hline
\multirow{1}{*}{Neurological} & Migraine & 1.6 [1.1, 2.4] {\it m} & 0.9 [0.8, 1.0]  & 1.80 [1.12, 2.87]  & 1122900 & 1390 & 208030 & 70 \\
 \hline
\multirow{1}{*}{Neoplasm/Tumor} & Neoplasm of stomach & 1.7 [0.8, 3.6]  & 0.4 [0.2, 0.6]  & 4.75 [1.21, 18.72]  & 35500 & 20 & 51160 & 20 \\
 \hline
\multirow{1}{*}{ENT issues} & Posterior rhinorrhea & 1.4 [0.7, 2.9]  & 0.5 [0.4, 0.6]  & 3.10 [1.12, 8.56]  & 96150 & 70 & 59130 & 20 \\
 \hline
\multirow{1}{*}{Inflammation} & Pharyngitis & 1.3 [0.9, 1.8]  & 0.7 [0.7, 0.8]  & 1.75 [1.10, 2.78]  & 1893860 & 1830 & 263480 & 70 \\
 \hline
			\end{tabular}
		}
		\caption{\textbf{Terms that exhibit higher co-morbidity with IPV in older women population compared to the background (BG) population.} For each term, we provide the co-morbidity scores for Senior and BG populations (after adjusted for selection bias), and the differential co-morbidity score. For each co-morbidity score, we report the following: The point estimate (odds ratio), 95\% augmented confidence interval (adjusted for FDR), and the corresponding co-morbidity level. The co-morbidity levels are abbreviated: H for high, M for moderate, and {\it m} for minor. All 20 reported terms are identified as differentially co-morbid with high confidence (this indicates that they exhibit higher association with IPV in older women population compared to the BG population in a statistically significant manner). See Supplementary Data 3 for a full list of terms identified as significant and their assigned categories.		
}
		\label{table:senior_vs_background}
	\end{table}	
\end{landscape}
